Catching a grown-up starfish planetary nebula II. Plasma analysis and central star properties of PC 22

After performing the morpho-kinematic analysis of the planetary nebula (PN) PC 22, we now present its nebular and stellar analysis. The plasma investigation relies on the novel use of a Monte Carlo analysis associated to the PyNeb code for the uncertainty propagation. The innermost region of the nebula shows electronic temperatures $T_{\rm e}$ $\approx$ 10,800~K using [NII] and $\approx$ 13,000 K using [OIII] and electronic densities $n_{\rm e}$ $\approx$ 600~cm$^{-3}$. We also used for the first time a Machine Learning Algorithm to calculate Ionisation Correction Factors (ICFs) specifically adapted to PC 22. This has allowed us to have pioneer ICFs for (S$^{+}$ + S$^{++}$)/O$^{++}$, Cl$^{++}$/O$^{++}$, and Ar$^{3+}$+Ar$^{4+}$, as well as a possible new determination for the total abundance of neon. The study of the stellar spectrum revealed the presence of broad emission lines consistent with a Wolf-Rayet-type [WR] classification and more precisely a [WO1]-subtype based on different qualitative and quantitative criteria. This classification is also coherent with the high stellar temperature derived from the reproduction of the ionization state of the gas with the Mexican Million Models database (3MdB) and the best fit model obtained with the NLTE model atmosphere code PoWR. PC 22 is therefore a new addition to the [WO1]-subtype PNe.

==> tab1_final.tex <==
\,[Ne~{\sc v}]                           & 3346 &           -        &           -        &    28.9$\pm$  1.7 &    37.9$\pm$  2.3&    41.0$\pm$  2.7 &    70.0$\pm$  4.5 &           -        &           -         \\
\,[Ne~{\sc v}]                           & 3426 &           -        &           -        &    84.1$\pm$  4.6 &   108.7$\pm$  6.0&    96.5$\pm$  5.6 &   159.8$\pm$  9.3 &           -        &           -         \\
\,[O~{\sc ii}]$\dagger$                  & 3727 &           -        &           -        &    18.9$\pm$  1.4 &    23.4$\pm$  1.7&    17.9$\pm$  1.7 &    27.3$\pm$  2.6 &           -        &           -         \\
\ion{He}{ii}+H10                         & 3798 &           -        &           -        &     4.5$\pm$  0.6 &     5.6$\pm$  0.7&     4.8$\pm$  0.4 &     7.2$\pm$  0.7 &           -        &           -         \\
\ion{He}{ii}+H9                          & 3835 &           -        &           -        &     9.9$\pm$  0.6 &    12.1$\pm$  0.7&     8.2$\pm$  0.6 &    12.1$\pm$  0.8 &           -        &           -         \\
\,[Ne~{\sc iii}]                         & 3869 &           -        &           -        &    61.7$\pm$  3.3 &    74.9$\pm$  4.0&    72.3$\pm$  3.9 &   105.9$\pm$  5.7 &           -        &           -         \\
\ion{He}{i}+H8$\dagger$                  & 3889 &           -        &           -        &     9.8$\pm$  0.7 &    11.8$\pm$  0.9&    10.9$\pm$  0.8 &    15.9$\pm$  1.1 &           -        &           -         \\
H$\epsilon$ $\dagger$                    & 3970 &           -        &           -        &    24.3$\pm$  1.4 &    29.0$\pm$  1.7&    29.3$\pm$  1.6 &    41.6$\pm$  2.3 &           -        &           -         \\
\,[S~{\sc ii}]                           & 4069 &           -        &           -        &     2.1$\pm$  0.2 &     2.4$\pm$  0.3&           -        &           -        &           -        &           -         \\
\ion{He}{ii}+H$\delta$                   & 4102 &           -        &           -        &    21.3$\pm$  1.2 &    24.8$\pm$  1.4&    23.0$\pm$  1.4 &    31.1$\pm$  1.8 &           -        &           -         \\
\ion{He}{ii}                            & 4200 &           -        &           -        &           -        &           -       &     1.7$\pm$  0.4 &     2.2$\pm$  0.5 &           -        &           -         \\
H$\gamma$                                & 4341 &           -        &           -        &    42.2$\pm$  2.3 &    46.8$\pm$  2.6&    44.0$\pm$  2.5 &    54.0$\pm$  3.0 &           -        &           -         \\
\,[O~{\sc iii}]                          & 4363 &           -        &           -        &    12.7$\pm$  0.8 &    14.0$\pm$  0.9&    13.2$\pm$  0.8 &    16.1$\pm$  1.0 &           -        &           -         \\
\ion{He}{i}                              & 4471 &           -        &           -        &     0.7$\pm$  0.3 &     0.8$\pm$  0.3&     1.3$\pm$  0.4 &     1.5$\pm$  0.5 &           -        &           -         \\
\ion{He}{ii}                             & 4542 &           -        &           -        &     3.0$\pm$  0.2 &     3.2$\pm$  0.2&     3.5$\pm$  0.3 &     3.9$\pm$  0.3 &           -        &           -         \\
\ion{N}{iii}                             & 4634 &           -        &           -        &     1.0$\pm$  0.2 &     1.0$\pm$  0.2&           -        &           -        &           -        &           -         \\
\ion{N}{iii}+\ion{O}{ii}                 & 4640 &           -        &           -        &     2.3$\pm$  0.3 &     2.4$\pm$  0.3&     2.2$\pm$  0.3 &     2.4$\pm$  0.4 &           -        &           -         \\
\ion{He}{ii}                             & 4686 &   112.8$\pm$ 14.4 &   120.9$\pm$ 15.4 &   120.8$\pm$  6.3 &   124.9$\pm$  6.5&   120.8$\pm$  6.4 &   129.0$\pm$  6.8 &   158.9$\pm$ 18.9 &   160.9$\pm$ 19.2  \\
\ion{He}{i}+[Ar~{\sc iv}]                & 4711 &           -        &           -        &    17.9$\pm$  1.1 &    18.4$\pm$  1.1&    18.6$\pm$  1.1 &    19.6$\pm$  1.2 &           -        &           -         \\
\,[Ne~{\sc iv}]                          & 4726 &           -        &           -        &     1.9$\pm$  0.3 &     1.9$\pm$  0.3&     2.5$\pm$  0.3 &     2.6$\pm$  0.4 &           -        &           -         \\
\,[Ar~{\sc iv}]                          & 4740 &           -        &           -        &    13.2$\pm$  0.8 &    13.5$\pm$  0.8&    14.1$\pm$  0.9 &    14.7$\pm$  1.0 &           -        &           -         \\
H$\beta$                                 & 4861 &   100.0$\pm$  9.0 &   100.0$\pm$  9.0 &   100.0$\pm$  5.2 &   100.0$\pm$  5.2&   100.0$\pm$  5.2 &   100.0$\pm$  5.2 &   100.0$\pm$ 13.8 &   100.0$\pm$ 13.8  \\
\,[O~{\sc iii}]                          & 4959 &   309.3$\pm$ 22.8 &   298.4$\pm$ 22.0 &   343.9$\pm$ 17.3 &   338.1$\pm$ 17.0&   362.3$\pm$ 18.3 &   350.3$\pm$ 17.7 &   431.0$\pm$ 33.0 &   428.2$\pm$ 32.8  \\
\,[O~{\sc iii}]                          & 5007 &  1070.5$\pm$ 60.9 &  1015.2$\pm$ 57.8 &  1027.0$\pm$ 51.6 &  1001.4$\pm$ 50.3&  1066.1$\pm$ 53.7 &  1014.6$\pm$ 51.1 &  1551.9$\pm$ 90.3 &  1537.1$\pm$ 89.5  \\
\ion{He}{ii}                             & 5411 &           -        &           -        &    10.0$\pm$  0.8 &     9.2$\pm$  0.7&    10.4$\pm$  0.8 &     8.9$\pm$  0.7 &           -        &           -         \\
\,[Cl~{\sc iii}]                         & 5518 &           -        &           -        &     1.5$\pm$  0.3 &     1.4$\pm$  0.3&     1.8$\pm$  0.4 &     1.5$\pm$  0.3 &           -        &           -         \\
\,[Cl~{\sc iii}]                         & 5538 &           -        &           -        &     1.2$\pm$  0.3 &     1.1$\pm$  0.2&     1.2$\pm$  0.4 &     1.0$\pm$  0.3 &           -        &           -         \\
\,[N~{\sc ii}]                           & 5755 &           -        &           -        &     0.8$\pm$  0.2 &     0.7$\pm$  0.2&     0.8$\pm$  0.4 &     0.6$\pm$  0.3 &           -        &           -         \\
\ion{He}{i}                              & 5876 &           -        &           -        &     4.9$\pm$  0.5 &     4.3$\pm$  0.4&     6.0$\pm$  0.5 &     4.6$\pm$  0.4 &           -        &           -         \\
\ion{He}{ii}                             & 6235 &           -        &           -        &     0.5$\pm$  0.2 &     0.4$\pm$  0.2&     0.8$\pm$  0.3 &     0.5$\pm$  0.2 &           -        &           -         \\
\,[O~{\sc i}]                            & 6300 &           -        &           -        &     1.0$\pm$  0.2 &     0.9$\pm$  0.2&     0.6$\pm$  0.4 &     0.5$\pm$  0.3 &           -        &           -         \\
\,[S~{\sc iii}]+\ion{He}{ii}             & 6312 &           -        &           -        &     7.9$\pm$  0.7 &     6.6$\pm$  0.6&     9.1$\pm$  0.7 &     6.4$\pm$  0.5 &           -        &           -         \\
\ion{He}{ii}                             & 6407 &           -        &           -        &     0.6$\pm$  0.2 &     0.5$\pm$  0.1&           -        &           -        &           -        &           -         \\
\,[Ar~{\sc V}]                           & 6435 &           -        &           -        &     3.5$\pm$  0.4 &     2.9$\pm$  0.3&     3.9$\pm$  0.4 &     2.7$\pm$  0.3 &           -        &           -         \\
\ion{He}{ii}                             & 6527 &           -        &           -        &     0.6$\pm$  0.3 &     0.5$\pm$  0.3&     1.0$\pm$  0.5 &     0.7$\pm$  0.3 &           -        &           -         \\
\,[N~{\sc ii}]                           & 6548 &           -        &           -        &    15.2$\pm$  0.9 &    12.5$\pm$  0.8&    18.9$\pm$  1.2 &    12.8$\pm$  0.8 &           -        &           -         \\
H$\alpha$                                & 6563 &   433.5$\pm$ 29.3 &   285.4$\pm$ 19.3 &   348.7$\pm$ 17.6 &   285.9$\pm$ 14.5&   421.8$\pm$ 21.5 &   285.4$\pm$ 14.5 &   307.3$\pm$ 26.8 &   285.0$\pm$ 24.9  \\
\,[N~{\sc ii}]                           & 6584 &           -        &           -        &    48.4$\pm$  2.6 &    39.6$\pm$  2.1&    53.5$\pm$  3.0 &    36.1$\pm$  2.0 &    51.1$\pm$ 15.3 &    47.3$\pm$ 14.2  \\
\ion{He}{i}$\dagger$                     & 6678 &           -        &           -        &           -        &           -       &     1.7$\pm$  0.4 &     1.1$\pm$  0.3 &           -        &           -         \\
\,[S~{\sc ii}]                           & 6716 &           -        &           -        &     9.6$\pm$  0.7 &     7.8$\pm$  0.6&    11.0$\pm$  0.9 &     7.2$\pm$  0.6 &           -        &           -         \\
\,[S~{\sc ii}]                           & 6731 &           -        &           -        &     9.1$\pm$  0.7 &     7.3$\pm$  0.6&    10.7$\pm$  0.8 &     7.0$\pm$  0.5 &           -        &           -         \\


==> tab1_final2.tex <==
\,[Ne~{\sc v}]                           & 3346 & 
                  -        &           -        & 
           28.9 $\pm$  2.3 &    38.9 $\pm$  3.1 & 
           41.0 $\pm$  4.1 &    55.4 $\pm$  5.5 & 
                  -        &           -        
        \\
\,[Ne~{\sc v}]                           & 3426 & 
                  -        &           -        & 
           84.1 $\pm$  4.6 &   111.3 $\pm$  6.1 & 
           96.5 $\pm$  6.2 &   128.1 $\pm$  8.2 & 
                  -        &           -        
        \\
\,[O~{\sc ii}]$\dagger$                  & 3727 & 
                  -        &           -        & 
           18.9 $\pm$  2.0 &    23.9 $\pm$  2.6 & 
           17.9 $\pm$  3.6 &    22.7 $\pm$  4.6 & 
                  -        &           -        
        \\
\ion{He}{ii}+H10                         & 3798 & 
                  -        &           -        & 
            4.5 $\pm$  2.6 &     5.7 $\pm$  3.3 & 
            4.8 $\pm$  5.2 &     6.0 $\pm$  6.5 & 
                  -        &           -        
        \\
\ion{He}{ii}+H9                          & 3835 & 
                  -        &           -        & 
            9.9 $\pm$  0.6 &    12.3 $\pm$  0.8 & 
            8.2 $\pm$  0.8 &    10.2 $\pm$  1.0 & 
                  -        &           -        
        \\
\,[Ne~{\sc iii}]                         & 3869 & 
                  -        &           -        & 
           61.7 $\pm$  3.1 &    76.3 $\pm$  3.8 & 
           72.3 $\pm$  3.7 &    89.6 $\pm$  4.6 & 
                  -        &           -        
        \\
\ion{He}{i}+H8$\dagger$                  & 3889 & 
                  -        &           -        & 
            9.8 $\pm$  0.5 &    12.1 $\pm$  0.6 & 
           10.9 $\pm$  0.7 &    13.5 $\pm$  0.8 & 
                  -        &           -        
        \\
H$\epsilon$ $\dagger$                    & 3970 & 
                  -        &           -        & 
           24.3 $\pm$  1.3 &    29.5 $\pm$  1.6 & 
           29.3 $\pm$  1.8 &    35.7 $\pm$  2.2 & 
                  -        &           -        
        \\
\,[S~{\sc ii}]                           & 4069 & 
                  -        &           -        & 
            2.1 $\pm$  0.5 &     2.5 $\pm$  0.6 & 
                  -        &           -        & 
                  -        &           -        
        \\
H$\delta$                                & 4102 & 
                  -        &           -        & 
           21.3 $\pm$  1.1 &    25.2 $\pm$  1.3 & 
           23.0 $\pm$  1.3 &    27.3 $\pm$  1.5 & 
                  -        &           -        
        \\
\ion{He}{ii}                             & 4200 & 
                  -        &           -        & 
                  -        &           -        & 
            1.7 $\pm$  0.7 &     1.9 $\pm$  0.9 & 
                  -        &           -        
        \\
H$\gamma$                                & 4341 & 
                  -        &           -        & 
           42.2 $\pm$  2.1 &    47.3 $\pm$  2.4 & 
           44.0 $\pm$  2.2 &    49.4 $\pm$  2.5 & 
                  -        &           -        
        \\
\,[O~{\sc iii}]                          & 4363 & 
                  -        &           -        & 
           12.7 $\pm$  0.7 &    14.2 $\pm$  0.7 & 
           13.2 $\pm$  0.7 &    14.7 $\pm$  0.8 & 
                  -        &           -        
        \\
\ion{He}{i}                              & 4471 & 
                  -        &           -        & 
            0.7 $\pm$  0.1 &     0.8 $\pm$  0.2 & 
            1.3 $\pm$  0.3 &     1.4 $\pm$  0.3 & 
                  -        &           -        
        \\
\ion{He}{ii}                             & 4542 & 
                  -        &           -        & 
            3.0 $\pm$  0.3 &     3.2 $\pm$  0.3 & 
            3.5 $\pm$  0.6 &     3.7 $\pm$  0.6 & 
                  -        &           -        
        \\
\ion{N}{iii}                             & 4634 & 
                  -        &           -        & 
            1.0 $\pm$  0.2 &     1.0 $\pm$  0.2 & 
                  -        &           -        & 
                  -        &           -        
        \\
\ion{N}{iii}+\ion{O}{ii}                 & 4640 & 
                  -        &           -        & 
            2.3 $\pm$  0.2 &     2.4 $\pm$  0.2 & 
            2.2 $\pm$  0.4 &     2.3 $\pm$  0.4 & 
                  -        &           -        
        \\
\ion{He}{ii}                             & 4686 & 
          112.8 $\pm$  9.8 &   120.9 $\pm$ 10.5 & 
          120.8 $\pm$  6.0 &   125.3 $\pm$  6.3 & 
          120.8 $\pm$  6.1 &   125.3 $\pm$  6.3 & 
          158.9 $\pm$ 17.7 &   160.8 $\pm$ 17.9 
        \\
\ion{He}{i}+[Ar~{\sc iv}]                & 4711 & 
                  -        &           -        & 
           17.9 $\pm$  0.9 &    18.5 $\pm$  0.9 & 
           18.6 $\pm$  1.0 &    19.1 $\pm$  1.0 & 
                  -        &           -        
        \\
\,[Ne~{\sc iv}]                          & 4726 & 
                  -        &           -        & 
            1.9 $\pm$  0.1 &     1.9 $\pm$  0.2 & 
            2.5 $\pm$  0.3 &     2.6 $\pm$  0.3 & 
                  -        &           -        
        \\
\,[Ar~{\sc iv}]                          & 4740 & 
                  -        &           -        & 
           13.2 $\pm$  0.7 &    13.5 $\pm$  0.7 & 
           14.1 $\pm$  0.7 &    14.5 $\pm$  0.8 & 
                  -        &           -        
        \\
H$\beta$                                 & 4861 & 
          100.0 $\pm$  5.9 &   100.0 $\pm$  5.9 & 
          100.0 $\pm$  5.0 &   100.0 $\pm$  5.0 & 
          100.0 $\pm$  5.0 &   100.0 $\pm$  5.0 & 
          100.0 $\pm$  7.9 &   100.0 $\pm$  7.9 
        \\
\,[O~{\sc iii}]                          & 4959 & 
          309.3 $\pm$ 15.7 &   298.4 $\pm$ 15.1 & 
          343.9 $\pm$ 17.2 &   337.5 $\pm$ 16.9 & 
          362.3 $\pm$ 18.1 &   355.4 $\pm$ 17.8 & 
          431.0 $\pm$ 22.1 &   428.4 $\pm$ 22.0 
        \\
\,[O~{\sc iii}]                          & 5007 & 
         1070.5 $\pm$ 53.8 &  1015.7 $\pm$ 51.1 & 
         1027.0 $\pm$ 51.3 &   999.1 $\pm$ 50.0 & 
         1066.1 $\pm$ 53.3 &  1037.0 $\pm$ 51.8 & 
         1551.9 $\pm$ 78.4 &  1538.1 $\pm$ 77.7 
        \\
\ion{He}{ii}                             & 5411 & 
                  -        &           -        & 
           10.0 $\pm$  0.5 &     9.1 $\pm$  0.5 & 
           10.4 $\pm$  0.5 &     9.5 $\pm$  0.5 & 
                  -        &           -        
        \\
\,[Cl~{\sc iii}]                         & 5518 & 
                  -        &           -        & 
            1.5 $\pm$  0.1 &     1.4 $\pm$  0.1 & 
            1.8 $\pm$  0.1 &     1.6 $\pm$  0.1 & 
                  -        &           -        
        \\
\,[Cl~{\sc iii}]                         & 5538 & 
                  -        &           -        & 
            1.2 $\pm$  0.1 &     1.1 $\pm$  0.1 & 
            1.2 $\pm$  0.2 &     1.1 $\pm$  0.2 & 
                  -        &           -        
        \\
\,[N~{\sc ii}]                           & 5755 & 
                  -        &           -        & 
            0.8 $\pm$  0.1 &     0.7 $\pm$  0.1 & 
            0.8 $\pm$  0.2 &     0.7 $\pm$  0.2 & 
                  -        &           -        
        \\
\ion{He}{i}                              & 5876 & 
                  -        &           -        & 
            4.9 $\pm$  0.3 &     4.3 $\pm$  0.2 & 
            6.0 $\pm$  0.4 &     5.1 $\pm$  0.3 & 
                  -        &           -        
        \\
\ion{He}{ii}                             & 6235 & 
                  -        &           -        & 
            0.5 $\pm$  0.1 &     0.4 $\pm$  0.1 & 
            0.8 $\pm$  0.2 &     0.6 $\pm$  0.2 & 
                  -        &           -        
        \\
\,[O~{\sc i}]                            & 6300 & 
                  -        &           -        & 
            1.0 $\pm$  0.1 &     0.8 $\pm$  0.1 & 
            0.6 $\pm$  0.1 &     0.5 $\pm$  0.1 & 
                  -        &           -        
        \\
\,[S~{\sc iii}]+\ion{He}{ii}             & 6312 & 
                  -        &           -        & 
            7.9 $\pm$  0.4 &     6.5 $\pm$  0.3 & 
            9.1 $\pm$  0.5 &     7.5 $\pm$  0.4 & 
                  -        &           -        
        \\
\ion{He}{ii}                             & 6407 & 
                  -        &           -        & 
            0.6 $\pm$  0.1 &     0.5 $\pm$  0.1 & 
                  -        &           -        & 
                  -        &           -        
        \\
\,[Ar~{\sc V}]                           & 6435 & 
                  -        &           -        & 
            3.5 $\pm$  0.2 &     2.8 $\pm$  0.2 & 
            3.9 $\pm$  0.2 &     3.2 $\pm$  0.2 & 
                  -        &           -        
        \\
\ion{He}{ii}                             & 6527 & 
                  -        &           -        & 
            0.6 $\pm$  0.2 &     0.5 $\pm$  0.2 & 
            1.0 $\pm$  0.4 &     0.8 $\pm$  0.4 & 
                  -        &           -        
        \\
\,[N~{\sc ii}]                           & 6548 & 
                  -        &           -        & 
           15.2 $\pm$  0.8 &    12.3 $\pm$  0.6 & 
           18.9 $\pm$  1.0 &    15.2 $\pm$  0.8 & 
                  -        &           -        
        \\
H$\alpha$                                & 6563 & 
          433.5 $\pm$ 23.4 &   286.3 $\pm$ 15.5 & 
          348.7 $\pm$ 17.4 &   280.7 $\pm$ 14.0 & 
          421.8 $\pm$ 21.1 &   338.8 $\pm$ 16.9 & 
          307.3 $\pm$ 23.4 &   286.3 $\pm$ 21.8 
        \\
\,[N~{\sc ii}]                           & 6584 & 
                  -        &           -        & 
           48.4 $\pm$  2.4 &    38.9 $\pm$  1.9 & 
           53.5 $\pm$  2.7 &    42.9 $\pm$  2.2 & 
           51.1 $\pm$ 10.4 &    47.5 $\pm$  9.7 
        \\
\ion{He}{i}$\dagger$                     & 6678 & 
                  -        &           -        & 
                  -        &           -        & 
            1.7 $\pm$  0.6 &     1.3 $\pm$  0.5 & 
                  -        &           -        
        \\
\,[S~{\sc ii}]                           & 6716 & 
                  -        &           -        & 
            9.6 $\pm$  0.5 &     7.6 $\pm$  0.4 & 
           11.0 $\pm$  0.6 &     8.7 $\pm$  0.4 & 
                  -        &           -        
        \\
\,[S~{\sc ii}]                           & 6731 & 
                  -        &           -        & 
            9.1 $\pm$  0.5 &     7.2 $\pm$  0.4 & 
           10.7 $\pm$  0.7 &     8.4 $\pm$  0.5 & 
                  -        &           -        
        \\
\hline 
c(H$\beta$) & & & 0.61$^{*}$ & & 0.32 & & 0.32 & & 0.10$^{*}$ \\
%\hline 
%H$\beta$/1e15 (erg/s/cm$^{2}$) &&0.447  & 1.802 & 16.690 & 34.628 &8.483  & 17.726 &0.227  & 0.288 \\
log H$\beta$ (erg/s/cm$^{2}$)  &&-15.35& -14.74 & -13.78& -13.46 &-14.07 & -13.75 &-15.64 & -15.54 \\


==> tab2_final2.tex <==
\,[Ne~{\sc v}]                      & 3345 &    44.08 $\pm$  3.88 \\
\,[Ne~{\sc v}]                      & 3426 &   114.56 $\pm$  6.69 \\
\,[O~{\sc ii}]$\dagger$             & 3727 &    25.72 $\pm$  3.29 \\
\ion{He}{ii}+H10                    & 3798 &     5.59 $\pm$  4.40 \\
\ion{He}{ii}+H9                     & 3835 &     9.55 $\pm$  0.78 \\
\,[Ne~{\sc iii}]                    & 3869 &    80.06 $\pm$  4.06 \\
\ion{He}{i}+H8$\dagger$             & 3889 &    12.82 $\pm$  0.71 \\
H$\epsilon$ $\dagger$               & 3969 &    36.94 $\pm$  2.05 \\
\,[S~{\sc ii}]                      & 4070 &     2.04 $\pm$  0.75 \\
H$\delta$                           & 4102 &    26.65 $\pm$  1.42 \\
\ion{He}{ii}                        & 4199 &     1.89 $\pm$  0.59 \\
H$\gamma$                           & 4341 &    48.40 $\pm$  2.44 \\
\,[O~{\sc iii}]                     & 4363 &    14.54 $\pm$  0.77 \\
\ion{He}{i}                         & 4472 &     0.93 $\pm$  0.21 \\
\ion{He}{ii}                        & 4542 &     3.63 $\pm$  0.44 \\
\ion{N}{iii}                        & 4633 &     0.61 $\pm$  0.21 \\
\ion{N}{iii}+\ion{O}{ii}            & 4642 &     1.27 $\pm$  0.28 \\
\ion{He}{ii}                        & 4686 &   127.87 $\pm$  6.40 \\
\ion{He}{i}+[Ar~{\sc iv}]           & 4712 &    18.95 $\pm$  0.97 \\
\,[Ne~{\sc iv}]                     & 4725 &     2.19 $\pm$  0.19 \\
\,[Ar~{\sc iv}]                     & 4740 &    14.37 $\pm$  0.74 \\
H$\beta$                            & 4862 &   100.00 $\pm$  0.00 \\
\,[O~{\sc iii}]                     & 4960 &   352.26 $\pm$ 17.61 \\
\,[O~{\sc iii}]                     & 5007 &  1050.15 $\pm$ 52.51 \\
\ion{He}{ii}                        & 5412 &     9.63 $\pm$  0.49 \\
\,[Cl~{\sc iii}]                    & 5519 &     1.49 $\pm$  0.09 \\
\,[Cl~{\sc iii}]                    & 5538 &     1.15 $\pm$  0.15 \\
\,[N~{\sc ii}]                      & 5755 &     0.77 $\pm$  0.12 \\
\ion{He}{i}                         & 5876 &     4.79 $\pm$  0.29 \\
\ion{He}{ii}                        & 6236 &     0.52 $\pm$  0.11 \\
\,[O~{\sc i}]                       & 6301 &     0.80 $\pm$  0.09 \\
\,[S~{\sc iii}]+\ion{He}{ii}        & 6312 &     7.20 $\pm$  0.38 \\
\ion{He}{ii}                        & 6407 &     0.47 $\pm$  0.17 \\
\,[Ar~{\sc V}]                      & 6436 &     3.02 $\pm$  0.17 \\
\ion{He}{ii}                        & 6527 &     0.66 $\pm$  0.25 \\
\,[N~{\sc ii}]                      & 6549 &    14.53 $\pm$  0.73 \\
H$\alpha$                           & 6563 &   316.28 $\pm$ 15.82 \\
\,[N~{\sc ii}]                      & 6584 &    41.52 $\pm$  2.08 \\
\ion{He}{i}$\dagger$                & 6680 &     2.35 $\pm$  0.36 \\
\,[S~{\sc ii}]                      & 6716 &     8.58 $\pm$  0.43 \\
\,[S~{\sc ii}]                      & 6731 &     8.17 $\pm$  0.46 \\
\hline 
c(H$\beta$) & & 0.28 \\
\hline 


==> table.tex <==
\hline \hline \\
Parameter & Mean &  Median &  Std & Ref\\ 
\hline \hline \\
Te [OIII] & 13219.6 & 13168.8 & 1152.2 & \\ 
Te [NII] & 10634.8 & 10651.0 & 1893.9 &  \\ 
ne [SII] & 592.9 & 422.1 & 662.7 &  \\ 
ne [Cl III] & 12094.4 & 2288.5 & 173142.5 &  \\ 
ne [Ar IV] & 1883.5 & 1338.6 & 1827.6 &  \\ 
log Ar$^{+3}$/H^+ & -5.8 & -5.8 & 0.1 & \\ 
log Ar$^{+4}$/H^+ & -6.1 & -6.1 & 0.2 & \\ 
log Cl$^{++}$/H^+ & -6.9 & -6.9 & 0.3 & \\ 
log He$^+$/H^+ & -1.7 & -1.7 & 0.1 & \\ 
log He$^{++}$/H^+ & -1.1 & -1.1 & 0.1 & \\ 
log N$^+$/H^+ & -5.1 & -5.2 & 0.3 & \\ 
log Ne$^{++}$/H^+ & -4.5 & -4.5 & 0.1 & \\ 
log Ne$^{+3}$/H^+ & -3.4 & -3.4 & 0.3 & \\ 
log Ne$^{+4}$/H^+ & -4.3 & -4.3 & 0.1 & \\ 
log O$^0$/H^+ & -6.0 & -6.0 & 0.4 & \\ 
log O$^+$/H^+ & -5.1 & -5.1 & 0.4 & \\ 
log O$^{++}$/H^+ & -3.8 & -3.8 & 0.1 & \\ 
log S$^{+}$/H^+ & -6.3 & -6.3 & 0.3 & \\ 
log S$^{++}$/H^+ & -4.9 & -4.9 & 0.4 & \\ 
log ICF(O$^+$ + O$^{++}$) & 4.31e-01 & 4.38e-01 & 6.66e-02 & ANN \\ 
log ICF(O$^+$ + O$^{++}$) & 4.84e-01 & 4.84e-01 & 5.31e-02 & KB94 \\ 
log ICF(O$^+$ + O$^{++}$) & 5.70e-01 & 5.71e-01 & 6.86e-02 & DIMS14 \\ 
log ICF(N$^+$/O$^+$) & -1.27e-02 & 2.55e-03 & 9.66e-02 & ANN \\ 
log ICF(N$^+$/O$^+$) & -5.73e-18 & 0.00e+00 & 3.00e-17 & KB94 \\ 
log ICF(N$^+$/O$^+$) & -1.35e-01 & -1.38e-01 & 1.16e-02 & DIMS14 \\ 
log ICF(Ne$^{++}$/O$^{++}$) & 1.46e-01 & 1.53e-01 & 6.76e-02 & ANN \\ 
log ICF(Ne$^{++}$/O$^{++}$) & -7.74e-18 & 0.00e+00 & 2.90e-17 & KB94 \\ 
log ICF(Ne$^{++}$/O$^{++}$) & 1.74e-01 & 1.69e-01 & 5.48e-02 & DIMS14 \\ 
log ICF(Ne$^{+2}$ + Ne$^{+4}$) & 2.47e-01 & 2.46e-01 & 3.88e-02 & ANN \\ 
log ICF(Ne$^{+2}$ + Ne$^{+4}$) & 1.76e-01 & 1.76e-01 & 5.55e-17 & KB94 \\ 
log ICF(Ne$^{+2}$ + Ne$^{+4}$) & 2.53e-01 & 2.54e-01 & 1.10e-02 & DIMS14 \\ 
log ICF(S$^+$ + S$^{++}$) & 3.08e-01 & 3.02e-01 & 9.39e-02 & ANN \\ 
log ICF(S$^+$ + S$^{++}$) & 4.39e-01 & 4.51e-01 & 1.12e-01 & KB94 \\ 
log ICF((S$^+$ + S$^{++}$)/O$^+$) & -1.58e+00 & -1.59e+00 & 1.22e-01 & ANN \\ 
log ICF((S$^+$ + S$^{++}$)/O$^+$) & -1.04e+00 & -1.05e+00 & 2.47e-01 & DIMS14 \\ 
log ICF(Cl$^{++}$/O$^{+}$) & -1.44e+00 & -1.44e+00 & 1.24e-01 & ANN \\ 
log ICF(Cl$^{++}$/O$^{+}$) & -1.01e+00 & -1.04e+00 & 2.70e-01 & DIMS14 \\ 
log ICF(Ar$^{+3}$+ Ar$^{+4}$) & 6.79e-02 & 7.58e-02 & 7.48e-02 & ANN \\ 
log He/H & -0.97 & -0.96 & 0.05 & ICF HeH \\ 
log O/H & -3.35 & -3.36 & 0.17 & ICF OH ANN \\ 
log O/H & -3.30 & -3.31 & 0.15 & ICF OH KB94 \\ 
log O/H & -3.21 & -3.22 & 0.15 & ICF OH DIMS14 \\ 
log N/H & -3.44 & -3.44 & 0.24 & ICF NO ANN \\ 
log N/H & -3.37 & -3.38 & 0.24 & ICF NO KB94 \\ 
log N/H & -3.42 & -3.43 & 0.23 & ICF NO DIMS14 \\ 
log Ne/H & -3.86 & -3.86 & 0.18 & ICF NeO ANN \\ 
log Ne/H & -3.82 & -3.83 & 0.14 & ICF NeH ANN \\ 
log Ne/H & -3.95 & -3.96 & 0.15 & ICF NeO KB94 \\ 
log Ne/H & -3.89 & -3.90 & 0.14 & ICF NeH KB94 \\ 
log Ne/H & -3.78 & -3.78 & 0.17 & ICF NeO DIMS14 \\ 
log Ne/H & -3.81 & -3.83 & 0.14 & ICF NeH DIMS14 \\ 
log S/H & -4.56 & -4.61 & 0.42 & ICF SH ANN \\ 
log S/H & -4.74 & -4.75 & 0.24 & ICF SO ANN \\ 
log S/H & -4.45 & -4.47 & 0.28 & ICF SH KB94 \\ 
log S/H & -4.06 & -4.07 & 0.29 & ICF SO DIMS14 \\ 
log Cl/H & -6.57 & -6.57 & 0.26 & ICF ClO ANN \\ 
log Cl/H & -6.00 & -6.02 & 0.22 & ICF ClO DIMS14 \\ 
log Ar/H & -5.59 & -5.59 & 0.15 & ICF ArH ANN \\ 
\hline \hline \\
